Parameterized Verification of Coverability in Well-Structured Broadcast Networks

Parameterized verification of coverability in broadcast networks with finite state processes has been studied for different types of models and topologies. In this paper, we attempt to develop a theory of broadcast networks in which the processes can be well-structured transition systems. The resulting formalism is called well-structured broadcast networks. We give an algorithm to decide coverability of well-structured broadcast networks when reconfiguration of links between nodes is allowed. Further, for various types of communication topologies, we also prove the decidability of coverability in the static case as well. We do this by showing that for these types of static communication topologies, the broadcast network itself is a well-structured transition system, hence proving the decidability of coverability in the broadcast network.

==> eptcsdata.tex <==
\providecommand{\firstpage}{133}
\providecommand{\publicationstatus}{A. Orlandini, M. Zimmermann (Eds.): 9th Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF'18)\\
EPTCS 277, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.277.10}{10.4204/EPTCS.277.10}}

